The complexity of linear-time temporal logic over the class of ordinals

We consider the temporal logic with since and until modalities. This temporal logic is expressively equivalent over the class of ordinals to first-order logic by Kamp's theorem. We show that it has a PSPACE-complete satisfiability problem over the class of ordinals. Among the consequences of our proof, we show that given the code of some countable ordinal alpha and a formula, we can decide in PSPACE whether the formula has a model over alpha. In order to show these results, we introduce a class of simple ordinal automata, as expressive as B\"uchi ordinal automata. The PSPACE upper bound for the satisfiability problem of the temporal logic is obtained through a reduction to the nonemptiness problem for the simple ordinal automata.

==> proof-lemma-nonemptiness-exptime.tex <==
 Let $\aautomaton$ be of the form $\triple{\abasis}{Q, I, F, \mathcal{F}}{\delta_{next},\delta_{lim}}$.
By Lemma~\ref{lemma-mainproperty}, $\aautomaton$ has an accepting run iff
$\aautomaton$ has an accepting run of length strictly less than $\omega^{\length{\abasis}+ 2}$.
Hence,
$\aautomaton$ has an accepting run iff 
either
(A) there are $\alocation_0 \in I$, $\alocation_f \in F$ and $E, A \subseteq \abasis$
such that $\triple{\alocation_0}{E,A}{\alocation_f} \in R_{\length{\abasis} + 2}'$
or (B) there are $\alocation_0 \in I$, $\alocation \in Q$ and $E, A \subseteq \abasis$
such that $\triple{\alocation_0}{E,A}{\alocation} 
\in R_{\length{\abasis} + 2}'$,  $\triple{\alocation}{E',A'}{\alocation} \in R_{\length{\abasis} + 2}'$
and $A' \in \mathcal{F}$.
(A) deals with accepting runs of length some successor ordinal 
\iflpar
(see Lemma~\ref{lemma-nonemptiness-one}(II))
\else
(see Lemma~\ref{lemma-nonemptiness-one})
\fi
whereas (B) deals with accepting runs of length some limit ordinal 
\iflpar
(see Lemma~\ref{lemma-nonemptiness-one}(III))
\else
(see Lemma~\ref{lemma-nonemptiness-three})
\fi
In order to check (A),  
it is sufficient to test for $\triple{\alocation_0}{E,A}{\alocation_f} \in I \times 
\powerset{\abasis}^2 \times
F$ whether 
$\triple{\alocation_0}{E,A}{\alocation_f} \in R_{\length{\aset} + 2}' \subseteq R_{\length{\aset} + 3}$.
A similar condition can be defined for (B).
Since $\length{Q}$ is in $\mathcal{O}(2^{\length{\abasis}})$, computing 
$R_{\length{\abasis}+ 3}$ takes
$\length{\abasis}+ 3$ 
steps that   
requires polynomial time in $\length{\aautomaton}$ and  exponential time
in $\length{\abasis}$, we obtain the desired result. Observe that we can take advantage of the fact 
that 
computing
the transitive closure of a relation and the maximal strongly connected components  can be done
in polynomial time in the size of the relations. 
 \qed
